An EF2X Allocation Protocol for Restricted Additive Valuations

We study the problem of fairly allocating a set of $m$ indivisible goods to a set of $n$ agents. Envy-freeness up to any good (EFX) criteria -- which requires that no agent prefers the bundle of another agent after removal of any single good -- is known to be a remarkable analogous of envy-freeness when the resource is a set of indivisible goods. In this paper, we investigate EFX notion for the restricted additive valuations, that is, every good has some non-negative value, and every agent is interested in only some of the goods. We introduce a natural relaxation of EFX called EFkX which requires that no agent envies another agent after removal of any $k$ goods. Our main contribution is an algorithm that finds a complete (i.e., no good is discarded) EF2X allocation for the restricted additive valuations. In our algorithm we devise new concepts, namely "configuration" and "envy-elimination" that might be of independent interest. We also use our new tools to find an EFX allocation for restricted additive valuations that discards at most $\lfloor n/2 \rfloor -1$ goods. This improves the state of the art for the restricted additive valuations by a factor of $2$.

==> Restrictive_Submodular_EFX.tex <==

In Section \ref{ef2x}, we presented an algorithm that finds an $\EFXX$ allocation which is almost non-wasteful. A natural question that arises is whether there exists $\EFXX$ allocations that are more efficient? 
In this section, we address this question: can we find an allocation that is Pareto efficient and satisfies $\EFXX$?  We answer this question in the negative: 
we show that guaranteeing both Pareto efficiency and $\EFXX$ is not possible. Indeed, our result is stronger: for any constant $c$ and any integer $k$, there are instances in which guaranteeing Pareto efficiency and a $c$ approximation of $\EFkX$ is not possible. We start by defining $\EFkX$ allocations. 

\begin{definition}\label{cefkxdef}
	An allocation $X = \langle \alloc_1, ... , \alloc_n \rangle$ is $\cEFkX$, if for all $i \neq j$ and every collection of $k$ distinct goods $g_1,g_2,\ldots,g_k \in \alloc_j$  we have 
	$
	v_i(\alloc_i) \geq c v_i(\alloc_j \setminus\{g_1,g_2,\ldots,g_k\}).
	$
\end{definition}

Roughgarden and Plaut \cite{plaut2020almost} give the following example with restricted additive valuations in which no $\EFX$ and Pareto efficient algorithm exists..

\begin{example}
	Let $\agents = \{1, 2\}$ and $\goods = \{\good, \good_1, \good_2\}$. The utility functions are shown in Table \ref{roughgarden}. For this example, in any $\PO$ allocation, $\good_1$ must be allocated to agent $1$ and $\good_2$ must be allocated to agent $2$. By symmetry, we assume without loss of generality that agent $1$ receives $\good$. We have, 
	\begin{align*}
	\util_2(\alloc_1) = \util_2(\good) = \util_2(\alloc_1 \backslash \{\good_1\}) &= 2, \\
	\intertext{and}
	\util_2(\alloc_2) &= 1. \\
	\intertext{Therefore,}
	\util_2(\alloc_1 \backslash \{\good_1\}) &> \util_2(\alloc_2).
	\end{align*}
	
	\begin{table}
		\centering
		\begin{tabular}{ c|c c c }
			&$\good$ & $\good_1$ & $\good_2$\\
			\hline
			$\util_1$& $2$ & $1$ & $0$\\
			$\util_2$& $2$ & $0$ & $1$\\
		\end{tabular}
		\caption{Counter example for $\EFX + \PO$ }
		\label{roughgarden}
	\end{table}
	
\end{example}		

We generalize this example and for any integer $k$ and any constant $c \leq 1$ and present an instance that admits no  $\cEFkX$ and Pareto efficient allocation.	

\begin{example}
	Let $\agents = \{1, 2\}$ and $\goods = \{\good, \good_1, \dots , \good_k, \good'_1, \dots , \good'_k\}$. Also let $\util_1(\good) = \util_2(\good) = (\frac{1}{c}+1)^k$, $\util_1(\good_i) = \util_2(\good'_i) = (\frac{1}{c}+1)^{i-1}$ for all $i \in [k]$ and  $\util_1(\good'_i) = \util_2(\good_i) = 0$ (see Table \ref{efkxcounter}). In any $\PO$ allocation, $\good_i$ must be allocated to agent $1$ and $\good'_i$ must be allocated to agent $2$ for all $i \in [k]$. Without loss of generality (by symmetry), assume agent $1$ receives $\good$. We have,
	\begin{align*}
	\util_2(\alloc_1) &= \util_2(\good) \\ 
	&= \util_2(\alloc_1 \backslash \{\good_1, \good_2, \dots , \good_k\}\}) \\ 
	&= (\frac{1}{c}+1)^k .
	\intertext{Also,}
	\util_2(\alloc_2) &= 1 + (\frac{1}{c}+1) + \dots + (\frac{1}{c}+1)^{k-1} \\
	&= c((\frac{1}{c}+1)^k-1). \\
	\intertext{Therefore,}
	c \util_2(\alloc_1 \backslash \{\good_1, \good_2, \dots , \good_k\}) &> \util_2(\alloc_2).
	\end{align*}
	Thus, the allocation is not $\cEFkX$.
	\begin{table}
		\centering
		\begin{tabular}{ c|c c c c c c c c c c}
			&$\good$ & $\good_1$ & $\good_2$ & $\dots$ & $\good_k$ & $\good'_1$ & $\good'_2$ & $\dots$ & $\good'_k$ &\\
			\hline
			$\util_1$& $(\frac{1}{c}+1)^k$ & $1$ & $\frac{1}{c}+1$ & $\dots$ & $(\frac{1}{c}+1)^{k-1}$ & $0$ & $0$ & $\dots$ & $0$ &\\
			$\util_2$& $(\frac{1}{c}+1)^k$ & $0$ & $0$  & $\dots$ & $0$ & $1$ & $\frac{1}{c}+1$ & $\dots$ & $(\frac{1}{c}+1)^{k-1}$ &\\
		\end{tabular}
		\caption{Counter example for $\cEFkX + \PO$}
		\label{efkxcounter}
	\end{table}
\end{example}		

%We show that guaranteeing both Pareto optimality and (even) a generalization of $\EFXX$
%called $\cEFkX$ is not always possible. Roughly speaking, for any $k \in \mathbb{N}$ and $c \leq 1$, $\cEFkX$ requires that no agent envies another agent after the removal of any $k$ goods up to the factor of $c$. We show that for any integer $k$ and any constant $c \leq 1$, there are instances for which guaranteeing both $\cEFkX$ and Pareto optimality at the same time is not possible. 

Therefore, in order to get a Pareto optimal allocation, we need to relax the notion of fairness. To this end, we introduce $\EFXp$ which is a natural relaxation of $\EFX$. Roughly speaking, an allocation $\alloc$ is $\EFXp$ if no agent $i$ envies another agent $j$ after the removal of any good from $\alloc_j$ which is of positive value for $i$. (Indeed, $\EFX$ was originally defined in this way the first time \cite{bibid}.) Finally, we propose an algorithm that guarantees both $\EFXp$ and Pareto optimality for any number of goods and agents.

%Throughout this section, we evaluate restricted additive valuations for two criteria:  $\EFXp$ (see Definition \ref{efxpdef}) and $\PO$ (see Definition \ref{POdef}) which are notions of fairness and efficiency respectively. 

%Our results in this section are as follows. First we show that for any integer $k$ and any constant $c$ \HA{$\leq 1$}, there are instances for which guaranteeing both $\cEFkX$ (see Definition \ref{cefkxdef}) and pareto optimality at the same time is not possible. Afterwards, we propose an algorithm that guarantees $\EFXp$ and $\PO$ for any number of goods and agents.
We start with the formal definition of $\cEFkX$ which is a generalization of $\EFX$.


\begin{definition} \label{POdef}
	An allocation $\alloc$ is Pareto optimal or $\PO$, if there is no other allocation $\alloc'$ such that $\forall i: \util_i(\alloc'_i) \geq \util_i(\alloc_i)$ and $\exists j: \util_j(\alloc'_j) > \util_j(\alloc_j)$.
\end{definition}


%In Lemma \ref{easyefx} we show that for this setting,  we can easily find an $\EFX^+$ allocation via a version of Envy-graph based allocation. 
Next, we formally define $\EFXp$ which is a relaxation of $\EFX$ and then present an algorithm that guarantees $\EFXp$ and Pareto optimality at the same time. 

\begin{definition}\label{efxpdef}
	An allocation $X = \langle \alloc_1, ... , \alloc_n\rangle$ is $\EFXp$ if for all agents $i$ and $j$, $\util_i(\alloc_i) \geq \util_i(\alloc_j \setminus \{g\})$ for all $g \in X_j$ such that $\util_i(\alloc_j \setminus \{g\}) < \util_i(\alloc_j)$.
\end{definition}

In order to describe our algorithm, we need to define \textit{tight graphs} tight-graph and \textit{free paths}.

\begin{definition}
	Given a partial-allocation $\allocs=\langle \alloc_1,\alloc_2,\ldots,\alloc_n \rangle$, the  tight-graph of $\alloc$ is constructed as following:
	
	\begin{enumerate}
		\item There is a node for each agent and for each good. 
		\item There is an edge from agent $\agent$ to good $\good$ if $\util_{\agent}(\good) = v({\good})$ and $\good \notin \alloc_{\agent}$.
		\item There is and edge from good $\good$ to agent $\agent$ if $\good \in \alloc_{\agent}$.
	\end{enumerate}
\end{definition}

\begin{definition}
	A path in the tight-graph is free if it ends with an unallocated good.
\end{definition}

\begin{observation}\label{freeobs}
	If $\good$ is unallocated and there is an agent $\agent$ such that $\util_\agent(\good) > 0$, then $\agent \rightarrow \good$ is a free path ending in $\good$.
\end{observation}

Let $p_1 < ... < p_k$ be all the different values of the goods, $\goods_\ell = \{\good \in \goods | v({\good}) = p_\ell \}$ for all $1 \le \ell \le k$ and $\graph_i$ be the tight-graph with respect to $\goods_\ell$. Algorithm \ref{efxalg} allocates goods in decreasing order of their values. Starting from $\ell=k$ until $\ell=1$, we consider the tight-graph $\graph_\ell$. As long as there is a free path, we consider the agent with minimum utility who is the start of a free path $F$. We augment $F$, i.e., we allocate each good in this path to the agent preceeding it in $F$. Afterwards, the number of unallocated goods decreases by one. In the end of the algorithm, if any good was remaining, we allocate them arbitrarily. By Observation \ref{freeobs}, these goods are of value $0$ to every agent.
\begin{algorithm}
	\caption{RestrictedAdditive$\EFXp$} \label{efxalg}
	Input: $N, M, V = (\util_1, ..., \util_n)$
	
	Output: allocation $\allocs = \langle\alloc_1, ... , \alloc_n\rangle$
	
	\begin{algorithmic}
		\State Let $p_1 < ... < p_k$ be all the different values of goods
		\State Let $\goods_\ell = \{\good \in \goods | v({\good}) = p_\ell \}$  for all $1 \leq \ell \leq k$
		\For {$\ell \leftarrow k$ to $1$}
		\State Let $\util_1(\alloc_1) \leq \util_2(\alloc_2) \leq ... \leq \util_n(\alloc_n)$
		\State Construct the tight-graph $\graph_\ell$ w.r.t. $\goods_\ell$
		\While {there is a free path }
		\State Let $\agent_0 = \argmin \{\util_{\agent}(\alloc_{\agent})| \exists$ free path $F = (\agent_0, \good_1, \agent_1, ..., \agent_{f-1}, \good_f)\}$ 
		\State $\alloc_{\agent_0} \leftarrow \alloc_{\agent_0} \cup \{\good_1\}$
		\For {$j \leftarrow 1$ to $f-1$}
		\State $\alloc_{\agent_j} \leftarrow (\alloc_{\agent_j} \backslash \{\good_j\}) \cup \{\good_{j+1}\} $
		\EndFor
		\State Update $\graph_\ell$
		\EndWhile
		\EndFor
		\State Allocate all the non-allocated goods arbitrarily
	\end{algorithmic}
\end{algorithm}

\begin{theorem} \label{easyefx}
	Algorithm \ref{efxalg} returns an $\EFXp$ and $\PO$ allocation.
\end{theorem}

We prove by induction that at any point during Algorithm \ref{efxalg}, the partial allocation is $\EFXp$. In order to do so, we first prove that another invariant holds throughout the algorithm. 

\begin{lemma}\label{invariantObs}
	Let $p_1 < ... < p_k$ be all the different values of the goods, $\goods_\ell = \{\good \in \goods | v({\good}) = p_\ell \}$ for all $1 \leq \ell \leq k$ and $\graph_\ell$ be the tight-graph with respect to $\goods_\ell$.
	At any point during Algorithm \ref{efxalg}, if agent $j$ is reachable from agent $i$ in $\graph_\ell$, then $\util_j(\alloc_j) - \util_i(\alloc_i) \leq p_\ell$. 
\end{lemma}

\begin{proof}
	We prove this lemma by induction. Before any good of value $p_\ell$ is allocated, the claim holds since $\graph_\ell$ is empty. \HA{$\graph_\ell$ is not empty but no agent is reachable from another agent.} Now assume that the claim holds before path $F = (\agent_0, \good_1, \agent_1, ..., \agent_{f-1}, \good_f)$ is augmented (induction hypothesis). Let $\alloc'$ be the new allocation. 
	
	We consider $4$ cases:
	\begin{itemize}
		\item{$i \in F$ and $j \in F$:} 	Note that $\util_{i_t}(\alloc'_{i_t}) = \util_{i_t}(\alloc_{i_t})$ for all $t \in \{1, 2, \ldots, f-1\}$ and $\util(\alloc'_{i_0}) = \util_{i_0}(\alloc_{i_0}) + p_\ell$. By the induction hypothisis, utility of the agents along this path for their own bundle is in $[\util_{i_0}(\alloc_{i_0}), \util_{i_0}(\alloc_{i_0}) + p_\ell]$ both before and after the augmentation. Thus, the claim holds when both $i \in F$ and $j \in F$. 
		
		\item{$i \in F$ and $j \notin F$:} If $j$ is reachable from $i$ after the augmentation, it was also reachable before it. By induction hypothesis, 
		$\util_j(\alloc_j) - \util_i(\alloc_i) \leq p_\ell$.
		Since $\util_j(\alloc'_j) = \util_j(\alloc_j)$ and $\util_i(\alloc'_i) \geq \util_i(\alloc_i)$, we have 
		$\util_j(\alloc'_j) - \util_i(\alloc'_i) \leq p_\ell$.
		
		\item{$i \notin F$ and $j \in F$:} \HA{For any $t \in \{0, 1, \ldots, f-1\}$, if} If $\agent_t$ is reachable from $j$, then either $\agent_t$ was reachable from $j$ before the augmentation, or $\good_{\ell+1}$ \HA{$\good_{t+1}$} was reachable from $j$ before the augmentation. In either case, there would be a free path $F'$ starting from $j$ and ending in $\good_f$. By the choice of $F$ for augmentation, $\util_{i_0}(\alloc_{i_0}) \leq \util_j(\alloc_j)$. Hence, 
		\begin{align*}
		\util_j(\alloc'_j) - \util_i(\alloc'_i)  \leq \util_{i_0}(\alloc_{i_0}) + p_\ell - \util_i(\alloc_i) \leq p_\ell.
		\end{align*}
		\item {$i \notin F$ and $j \notin F$:} If $j$ is reachable from $i$ after the augmentation, it was also reachable before the augmentation. By the induction hypothesis and the fact that $\util_i(\alloc_i) = \util_i(\alloc'_i)$ and $\util_j(\alloc_j) = \util_j(\alloc'_j)$, the claim holds.
	\end{itemize}
\end{proof} 

Now we are ready to prove Lemma \ref{easyefx}.

\begin{proof}%[Lemma \ref{easyefx}]
	The proof is by induction. In the beginning of the the algorithm, before any good is allocated, the allocation is obviously $\EFXp$. Now assume that the allocation is $\EFXp$ before the path $F = (\agent_0, \good_1, \agent_1, ..., \agent_{f-1}, \good_f)$ is augmented (induction hypothesis). Let $\alloc'$ be the new allocation. Assume $\alloc'$ is not $\EFXp$. Hence there are agents $i$ and $j$ and a good $\good \in \alloc_j$ such that $\util_i(\alloc'_j) > \util_i(\alloc'_j \backslash \{\good\}) > \util_i(\alloc'_i)$.
	
	Since $j$ is reachable from $i$, by Lemma \ref{invariantObs},
	\begin{align*}
	\util_j(\alloc_j) &\leq \util_i(\alloc_i) + p_\ell. \\
	\intertext{	Note that the way we allocated the goods, all the agents have non-zero utility for all the goods in their bundle. This means, }
	\util_j(\alloc'_j) &\geq \util_i(\alloc'_j). \\
	\intertext{	Since we allocate goods in non-increasing order of their innate \HA{inherent} value, }
	\util_i(\good) &\geq p_\ell. \\
	\intertext{	Hence, we have,}
	\util_i(\alloc'_j \backslash \{\good\}) &= \util_i(\alloc'_j) - \util_i(\good) \\
	&\leq \util_j(\alloc'_j) - \util_i(\good).
	\end{align*}
	Now we consider two cases:
	\begin{itemize}
		\item {$j \neq i_0$:} In this case, $\util_j(\alloc_j) = \util_j(\alloc'_j)$. Hence we have,
		\begin{align*}
		\util_j(\alloc'_j) - \util_i(\good) 
		&= \util_j(\alloc_j) - \util_i(\good) \\
		&\leq \util_i(\alloc_i) + p_\ell - \util_i(\good) \\
		&\leq \util_i(\alloc_i).
		\end{align*}
		\item{$j = i_0$:} In this case, one of $j$ or $\good_1$ was reachable from $i$ before the augmentation which means that a free path $F'$ starting from $i$ existed. By the choice of $F$ for augmentation, we have $\util_i(\alloc_i) \geq \util_j(\alloc_j)$.  Therefore,
		\begin{align*}
		\util_j(\alloc'_j) - \util_i(\good) 
		&= \util_j(\alloc_j) + p_\ell - \util_j(\good) \\
		&\leq \util_i(\alloc_i) + p_\ell - \util_i(\good) \\
		&\leq \util_i(\alloc_i).
		\end{align*}
	\end{itemize}
	So there are no such agents $i$ and $j$ and allocation $\allocs'$ is $\EFXp$.
	
	Now we prove pareto optimality of the output. We prove that the result has maximum social welfare and therefore is pareto optimal. Let $\agents_\good$ be the set of agents $\agent$ for whom $\util_\agent(\good) = v(\good$). The maximum social welfare can be obtained when $\good$ is allocated to an agent in $\agents_\good$ for all $\good$ with $\agents_\good \neq \emptyset$. By Observation \ref{freeobs}, if $\agents_\good \neq \emptyset$, then there is a free path ending in $\good$. Therefore $\good$ is allocated when augmenting a free path $F$ and not in the end of the algorithm. Note that augmenting any free path, allocates and reallocates the good $h$ in it to the agent who values it at $v(h)$.  Hence, in the end of the algorithm, the utility of $\good$ is $v(\good)$ for its owner. 
\end{proof}



==> U0.tex <==
\subsubsection*{Rule $\mathsf{U}_0$} 
We start by rule $\textsf{U}_0$ which is our most basic rule. Roughly speaking, this rule states that if we could allocate a good to a source such that no agent envies this source after the allocation%,node without violating the $\EFX$ property
, we do so. %\HA{The precondition is stronger than this. No one should envy the source.} 
In the following, you can find an overview of this updating rule. 

\vspace{0.5cm}
\begin{tcolorbox}[%colback=blue!5,coltitle=blue!50!black,colframe=blue!25,
	title= \textbf{Rule U$_0$}]
	%Input: allocation $\allocs$
	
	Preconditions:\label{pre1}
	\begin{itemize}
		\item $X$ is $\EFX$ and almost non-wasteful. 
		\item %$\exists \good \in P, s \in S_{\allocs}$ s.t. $\forall i \in \agents \backslash \{s\}: \util_i(\alloc_i) \geq \util_i(\alloc_s \cup \{\good\})$
		There exists a good $ \good \in P$ and a source $i$ such that no agent $j \neq i$ envies $\alloc_i \cup \{\good\}$. 
	\end{itemize}
%	Output: 
%	\begin{itemize}
%	\item  $\alloc'_s = \alloc_s \cup \{\good\}.$ 
%	\item $\forall i \in \agents \backslash \{s\}: \alloc'_i = \alloc_i.$
%	\end{itemize}
	Guarantees:
	\begin{itemize}
		\item $X'$ is $\EFX$ and almost 
		non-wasteful.
		\item $\Phi(X')\lexlarger \Phi(X)$.
	\end{itemize}
\end{tcolorbox}
\vspace{0.5cm}

\paragraph{Rule $\mathsf{U}_0$:}
If there exists a good $\good \in P$ and a source $i$ such that no agent $j \neq i$ envies $\alloc_i \cup \{\good\}$, allocate $\good$ to $i$. %Formally,
%we set $\alloc'_s = \alloc_s \cup \{\good\}$ and for all $\agent \neq s$ we set $\alloc'_\agent = \alloc_\agent$. \HA{Do we still need this?}

\begin{observation}\label{main0}
	Let $X'$ be the allocation after updating $X$ via Rule $\textsf{U}_0$. Then, $X'$ is $\EFX$ and almost non-wasteful.
\end{observation}

\begin{lemma}\label{U0.3}
Rule $\textsf{U}_0$ is $\Phi$-improving.
\end{lemma}
\begin{proof}
	We consider two cases:
	\begin{itemize}
		\item If $\util_i(\good) = 0$, then $\graph_{\allocs'} = \graph_\allocs$ and thus, $S_{\alloc'} = S_\alloc$. We also have $\util_j(\alloc_j) = \util_j(\alloc'_j)$. Moreover, 
		$$\bigcup_{j \notin S_{\alloc'}} \alloc'_j = \bigcup_{j \notin S_{\alloc}} \alloc_j$$
		and
		$$\bigcup_{j \in S_{\alloc'}} \alloc'_j = \bigcup_{j \in S_{\alloc}} \alloc_j \cup \{\good\}.$$
		Therefore, 
		$$\sum_{j \in S_{\alloc'}} |\alloc'_j| = \sum_{j \in S_\alloc} |\alloc_j|+1$$ 
		and $\Phi(\allocs') \lexlarger \Phi(\allocs)$. 
		\item If $\util_i(\good) = \valu(\good)$ we have  $\util_i(\alloc'_i) > \util_i(\alloc_i)$, and for every $j \neq i$ we have $\util_j(\alloc'_j) = \util_j(\alloc_j)$. Therefore, if $S_{\allocs'} \backslash S_\allocs = \emptyset$,  Lemma \ref{lex1} implies that $\Phi(X')>\Phi(X)$.
		Otherwise let $j \in S_{\allocs'} \backslash S_\allocs$ be a source node in $\graph_{\allocs'}$. Since $j$ is not a source in $G_X$ and agent $i$ is the only agent whose valuation is improved after applying $\mathsf{U}_0$, agent $i$ envies $j$ under $X$. 
%		The envy-edges that are removed from $\graph_\allocs$ must be from $i$ to some other agent. Therefore, $i$ envies $j$ under $\allocs$. 
By Lemma \ref{sources are min}, we have $\util_j(\alloc'_j) > \util_i(\alloc_i) $. This, together with Lemma \ref{lex2} implies 
		$
		\Phi(X') \lexlarger \Phi(X). 
		$ 
	\end{itemize}
\end{proof}

==> U2-updated.tex <==
\subsubsection*{Rule $\mathsf{U}_2$}
Similar to Rule $\mathsf{U}_0$, our goal  in Rule $\mathsf{U}_2$  is to allocate some of the unallocated goods to some sources. More precisely, in this rule we find a \textit{champion cycle} in $H_\alloc$ as defined in Definition \ref{champion cycle} and update the allocation through this cycle.

\begin{definition}\label{champion cycle}
	For allocation $\alloc$, we call a cycle $C$ of $H_\alloc$ a \textit{champion cycle}, if for every champion edge $i \xrightarrow[]{g} j$ in $C$, agent $j$ is a source agent.
	Additionally, for every two champion edges of $C$ with labels $g$ and $g'$, we have that $g\neq g'$.
	%\HA{For any such cycle $C$, let $S_C$ be the set of its source agents.}
\end{definition}
In the following, you can find an overview of $\mathsf{U}_2$.
\vspace{0.5cm}
\begin{tcolorbox}[%colback=blue!5,coltitle=blue!50!black,colframe=blue!25,
	title= \textbf{Rule U$_2$}]
	%Input: allocation $\allocs$
	
	Preconditions:\label{pre1}
	\begin{itemize}
		\item $X$ is $\EFX$ and almost non-wasteful. 
		\item There exists a \textit{champion cycle} $C$ in $H_{\allocs}$.
	\end{itemize}
	Guarantees:
	\begin{itemize}
		\item $X'$ is $\EFX$ and almost 
		non-wasteful.
		\item $\Phi(X'){\lexlarger} \Phi(X)$.
	\end{itemize}
\end{tcolorbox} 
\vspace{0.5 cm}

\paragraph{Rule $\mathsf{U}_2$:} If there exists a \textit{champion cycle} $C$ in $H_{\allocs}$, we update $\allocs$ as follows:
\begin{itemize}
	\item for every envy edge $i \rightarrow j\in C$, set $\allocs'_{i} = \allocs_{j}$,
	\item for every champion edge $i \xrightarrow[]{g} j \in C$, set $\allocs'_i = \champset{\allocs_j \cup \{g\}}{i}$,
	\item for every agent $j \notin C$, let $\alloc'_j=\alloc_j$.
\end{itemize}

\begin{observation}\label{utility Change}
	Let $\alloc'$ be the allocation after updating $\alloc$  via Rule $\textsf{U}_2$. Then, $\util_i(\alloc'_i) > \util_i(\alloc_i)$ for all $i \in C$ and $\util_i(\alloc'_i) = \util_i(\alloc_i)$ for all $i \notin C$.
\end{observation}
\begin{proof}
	For $i \notin C, \alloc'_i = \alloc_i$ and therefore, $\util_i(\alloc'_i) = \util_i(\alloc_i)$. Let $T_C$ be the set of the champion agents in $C$. Any agent $i \in C \setminus T_C $ receives a bundle she envied. Therefore, $\util_i(\alloc'_i) > \util_i(\alloc_i)$. Moreover, any agent $i \in T_C$ is a champion of the bundle she receives. Thus, by definition, $\util_i(\alloc'_i) > \util_i(\alloc_i)$.
\end{proof}


\begin{lemma}\label{main2}
	Let $X'$ be the allocation after updating $X$ via Rule $\textsf{U}_2$. Then, $X'$ is $\EFX$ and almost non-wasteful.
\end{lemma}
\begin{proof}
	For any agent $i$, we prove that no agent strongly envies $\alloc'_i$ under allocation $\alloc'$. Note that for any bundle $\alloc'_i$, either we have $\alloc'_i = \alloc_j$ or we have $\alloc'_i = \champset{\alloc'_j \cup \{\good\}}{i}$ for some agent $j$ and some good $\good \in P(\alloc)$. Consider these two cases:
	\begin{itemize}
		\item $\alloc'_i = \alloc_j$ for some agent $j$: by Observation \ref{utility Change}, for every agent $\ell$ we have $\valu_\ell(\alloc'_\ell) \geq \valu_\ell(\alloc_\ell)$. Therefore, if agent $\ell$ did not strongly envy $\alloc_j$ before the update, she does not strongly envy $\alloc'_i$ after the update either.  
		\item $\alloc'_i = \champset{\alloc'_j \cup \{\good\}}{i}$ for some agent $j$ and some good $\good \in P(\alloc)$: by definition, no agent strongly envies $\champset{\alloc_j \cup \{\good\}}{j}$ under $\alloc$. By Observation \ref{utility Change}, for every agent $\ell$ we have $\valu_\ell(\alloc'_\ell) \geq \valu_\ell(\alloc_\ell)$. Hence, $\ell$ does not strongly envy $\alloc'_i$ either.
	\end{itemize}
	To show that $\alloc'$ is almost non-wasteful, note that by Observations \ref{i envy j likes full bundle} and \ref{i envies y likes full bundle} for all agents $i \in C$, $\util_i(\alloc'_i) = \valu(\alloc'_i)$.
	Also, since $\alloc$ is almost non-wasteful, for all agents $i \notin S_\alloc$, $\util_i(\alloc_i) = \valu(\alloc_i)$. 
	Since $\alloc'_i = \alloc_i$ for all $i \notin C$, we only need to argue that for all $i \in S_\alloc \setminus C$, $i \in S_{\alloc'}$. Let $i \in S_\alloc \setminus C$. We know $\alloc'_i = \alloc_i$ and for all agents $j$, $\util_j(\alloc_j) \geq \util_j(\alloc_i)$. Together with Observation \ref{utility Change} we have
	$$\util_j(\alloc'_j) \geq \util_j(\alloc_j) \geq \util_j(\alloc_i).$$
	Therefore, no agent envies $i$ under allocation $\alloc'$ and $i \in S_{\alloc'}$.
\end{proof}

\begin{observation}\label{new sources}
	%Let $\alloc'$ be the allocation after updating $\alloc$  via Rule $\textsf{U}_2$. Then, for any agent $i \in S_{\alloc'}$, either $i \in S_{\alloc}$ or $i$ is reachable from some source in $C$. \HA{It is confusing. We are talking about reachability in $G_X$ but agents in $C$. Alternative: ... is in $G_\alloc$ reachable from some agent in $S_\alloc \cap C$.}
	Let $\alloc'$ be the allocation after updating $\alloc$  via Rule $\textsf{U}_2$. Then, for any agent $i \in S_{\alloc'}$, either $i \in S_{\alloc}$ or $i$ is  reachable in $G_\alloc$ from some agent in $S_\alloc \cap C$.
\end{observation}
\begin{proof}
	Let $i \in S_{\alloc'} \setminus S_\alloc$. If $\alloc'_i \neq \alloc_i$, then $i \in C$ and therefore (by definition of champion cycles), $i$ is reachable from  some agent in $S_\alloc \cap C$.
	Now assume $\alloc'_i = \alloc_i$. Under allocation $\alloc$, some agent $j$ envies $\alloc_i$. Since $j$ does not envy $i$ under $\alloc'$, we have,
	\begin{align*}
		\util_j(\alloc'_j) &\geq \util_j(\alloc'_i) \\
		&= \util_j(\alloc_i) \\
		&> \util_j(\alloc_j).
	\end{align*}
	Therefore $\alloc'_j \neq \alloc_j$ and $j \in C$. Thus, $i$ is reachable from some agent in $S_\alloc \cap C$.
\end{proof}

\begin{lemma}\label{potential func u2}
	Rule $\textsf{U}_2$ is $\Phi$-improving.
\end{lemma}
\begin{proof}
	We use Observation \ref{lex2} to prove this lemma. First note that by Observation \ref{utility Change}, $\valu_i(\allocs'_i)\geq \valu_i(\allocs_i)$ for all agents $i$	. 
	Let $i \in C$ be a source that minimizes $\util_i(\alloc_i)$, i.e, 
	$$i = \argmin_{j \in S_\alloc \cap C}\{\util_j(\alloc_j)\}.$$
	By Observation \ref{utility Change}, $\util_i(\alloc'_i) > \util_i(\alloc_i)$. Also, by Observation \ref{new sources}, for any agent $j \in S_{\alloc'} \setminus S_{\alloc}$, $j$ is reachable from some source $\ell$ in $C$. We have
	\begin{align*}
		\util_j(\alloc'_j) &\geq \util_j(\alloc_j) &\hbox{Lemma \ref{utility Change}}\\
		&> \util_\ell(\alloc_\ell) &\hbox{Lemma \ref{sources are min}}\\
		&\geq \util_i(\alloc_i). &\hbox{by the choice of $i$}
	\end{align*}
	Thus, by Lemma \ref{lex2}, $\Phi(\alloc') \lexlarger \Phi(\alloc)$.
\end{proof}


==> U2.tex <==
\subsubsection*{Rule $\mathsf{U}_2$}
The goal of this update rule is to remove a certain type of cycle in champion graph.
\vspace{0.5 cm}

\begin{tcolorbox}[%colback=blue!5,coltitle=blue!50!black,colframe=blue!25,
	title= \textbf{Rule U$_2$}]
	%Input: allocation $\allocs$
	
	Preconditions:\label{pre1}
	\begin{itemize}
		\item $X$ is $\EFX$ and almost non-wasteful. 
		\item $C$ is a cycle from $H_{\allocs}$ as defined in Definition \ref{champion cycle}
	\end{itemize}
	Guarantees:
	\begin{itemize}
		\item $X'$ is $\EFX$ and almost
		non-wasteful.
		\item $\Phi(X')> \Phi(X)$.
	\end{itemize}
\end{tcolorbox} 
\vspace{0.5 cm}


\begin{definition}\label{champion cycle}
	Let $H_{\alloc}$ be the champion graph of $\allocs$. We call $C$ a \textit{champion cycle} if for every champion edge $i \xrightarrow[]{g} j$, $j$ is a source agent, and $i$ is champion of $\allocs_j \cup \{g\}$ where $g\in P_{\allocs}$. For any such cycle $C$, let $T_C$ be the set of its champion agents and $S_C$ be the set of its source agents. \HA{We should also mention the labels are different.}
\end{definition}

\paragraph{Rule $\mathsf{U}_2$:} If there exists a \textit{champion cycle} in $H_{\allocs}$, we define $\allocs'$ as follows:
\begin{itemize}
	\item Remove envy edges: For every envy edge $i \rightarrow j\in C$, set $\allocs'_{i} = \allocs_{j}$, 
	  \item Remove champion edges: For every champion edge $i \xrightarrow[]{g} j \in C$, set $\allocs'_i = \champset{\allocs_j \cup \{g\}}{i}$,
	  \item Leave other agents unchanged: For every agent $j$ not in $C$, let $\alloc'_j=\alloc_j$.
\end{itemize}

\begin{observation}\label{utility Change}
	After applying Rule $\textsf{U}_2$, the values of agents in $C$ strictly increases, and the remaining agents keep the same value as in $\alloc$.
\end{observation}
\begin{proof}
	The bundles of agents outside of $C$ do not change. Any agent in $C-T_C$ \HA{$C \setminus T_C$ (fix it everywhere.)} receives a bundle they envied. Therefore, their value strictly increases. Moreover, agents of $T_C$ receive their \edit{top set} of the bundle they were champion of, so per definition of champion their value strictly increases.
\end{proof}

\begin{observation}\label{new sources}
	Let $\alloc'$ be the allocation after updating $\alloc$  via Rule $\textsf{U}_2$. Then, $S_{\alloc'}\subseteq S_{\alloc}\cup (\underset{s\in S_C}{\bigcup} R_{s})$. 
	\HA{This is not accurate. $R_{s}$ is not all the vertices reachable from $s$ but also depends on the ordering of the sources. What you mean is that all sources in $\alloc'$ are reachable from $S_C$ or are in $S_\alloc$. There is no reference to this lemma.}
\end{observation}
\begin{proof}
	First, note that according to Observation \ref{utility Change}, values of agents in $S_{\alloc}\backslash S_C$ do not change, and values of every other agent either remains the same or increases. Agents in $S_{\alloc}\backslash S_C$ were source vertices, so there is no envy edge to them in $G_{\alloc}$. Moreover, since no agent's value decreases in $\alloc'$, no new agent envies a member of $S_{\alloc}\backslash S_C$. Therefore, these agents remain source agents in $G_{\allocs'}$. \HA{We do not need the first paragraph.}
	
	Next, note that in order for an agent not in $S_{\alloc}$ to become a source vertex in $\alloc'$, there needs to be an envy path from some member of $C$ to such agent in $G_{\alloc}$. This is because the only agents who could envy less agents after this update rule are those whose values have increased. This shows that such new source agent should be a member of $\underset{s\in S_C}{\bigcup} R_{s}$. This concludes the proof of Observation \ref{new sources}.
\end{proof}

\begin{lemma}\label{pareto}
	Let $\alloc'$ be the allocation after updating $\alloc$ via Rule  $\textsf{U}_2$. Then, $\alloc'$ is almost non-wasteful.
\end{lemma}
\begin{proof}
	For agents $i\in C-T_C$, since they receive the bundle they envy, according to Observation \ref{i envy j likes full bundle}, we have that $\valu_i(\allocs'_i)=\valu(\alloc'_{i})$. For agents $i\in T_C$, since they are champion of some bundle,their receiving bundle should be such that no agent envies them. If there exists a good $g\in\allocs'_i$ for which $\valu_i(\{g\})=0$, then $i$ herself strongly envies this bundle. Hence, we have $\valu_i(\alloc'_i)=\valu(\alloc'_i)$. This concludes proof of Lemma \ref{pareto}. \HA{What about other sources?}
\end{proof}


\begin{observation}\label{envy agents}
	Let $\alloc'$ be the allocation after updating $\alloc$ via Rule  $\textsf{U}_2$. Then no agent in $C-T_C$ strongly envies some other agent.
\end{observation}
\begin{proof}
	Consider an agent $i\in C-T_C$, and assume that they strongly envy some other agent $j$. Now $j$ can be in $3$ different groups: $[n]-C$, $C-T_C$ or $T_C$. If $j\in [n]-C$, note that value of $j$ has not changed, and value of $i$ has increased. Therefore, if $i$ strongly envies $j$ in $\alloc'$, then so does she in $\alloc$ which is a contradiction. If $j\in C-T_C$, there exists some agent $k\in C$ where $\alloc'_j=\alloc_k$. If $i$ strongly envies $j$, then $i$ strongly envies $\alloc_k$. Now note that value of $i$ has increased in $\alloc'$. This means that $i$ strongly envies $k$ in $\alloc$, which is a contradiction. If $j\in T_C$, for each member of $T_C$ we have the guarantee that they are champion of some set $\alloc_k\cup\{g\}$. By definition of champion, there exists no other agent that strongly envies the top set they receive. Hence, $i$ cannot strongly envy $j$ even with her bundle in $\alloc$.
\end{proof}


\begin{observation}\label{champ agents}
	Let $\alloc'$ be the allocation after updating $\alloc$ via Rule  $\textsf{U}_2$. Then no agent in $T_C$ strongly envies some other agent.
\end{observation}
\begin{proof}
		Consider an agent $i\in T_C$ and let $j$ be some agent that $i$ strongly envies. If $j\in S-T_C$, there exists some agent $k\in C$ for which $\alloc'_j=\alloc_k$. Since value of $i$ strictly increases, if $i$ strongly envies $j$ in $\alloc'$, then she strongly envies $k$ in $\alloc$, which is a contradiction. If $j \in T_C$, there exists a source agent $k$ and a good $g$ for which $j$ is champion of $\alloc_{k}\cup\{g\}$. Because of this property, we know that $i$ with $\allocs_i$ does not strongly envy $\alloc'_j$. Moreover, $\valu_i(\alloc'_i)>\valu_i(\alloc_i)$. Therefore, $i$ cannot strongly envy $j$ in $\alloc'$. If $j\in [n]-C$, value of agents in $[n]-C$ has not changed, while value of $i$ has increased in $\alloc'$. This means that if $i$ strongly envies $j$ in $\alloc'$, it must be that $i$ envies $j$ in $\alloc$ as well which is a contradiction.
\end{proof}


\begin{observation}\label{others}
	Let $\alloc'$ be the allocation after updating $\alloc$ via Rule  $\textsf{U}_2$. Then no agent in $[n]-C$ strongly envies some other agent.
\end{observation}
\begin{proof}
	Consider an agent $i\in [n]-C$ and let $j$ be some agent $i$ strongly envies. If $j\in [n]-C$, note that the allocation of neither $i$ nor $j$ has changed in $\alloc'$. This means if $i$ strongly envies $j$ in $\alloc'$, they should do so in $\alloc$ as well, which is a contradiction. If $j\in C-T_C$, for any such agent $j$, there exists $k\in C$ where $\alloc'_j=\alloc_k$. If $i$ strongly envies $j$ in $\alloc'$, then $i$ strongly envies $k$ in $\alloc$, which is a contradiction. If $j \in T_C$, $j$ is champion of some bundle $\alloc_k\cup\{g\}$. By definition, no agent strongly envies them in $\alloc$. Since allocation of agent $i$ does not change in $\alloc'$, they still cannot strongly envy champion agents in $\alloc'$.
\end{proof}

\HA{We do not need the last $3$ observations. Simple argument: No agent is worse off. Therefore, no agent envies any bundle that already existed under $\alloc$. Also by definition, no agent strongly envies champion bundles ($\champset{.}^{i}$). All the bundles under $\alloc'$ are of these two types.}



\begin{lemma}\label{efx}
	Let $\alloc'$ be the allocation after updating $\alloc$ via Rule  $\textsf{U}_2$. Then, $\alloc'$ is $\EFX$.
	
\end{lemma}

\begin{proof}
	Let $i$ be an agent in $[n]$. If i$C-T_C$, $i\in T_C$ or $i\in [n]-C$she does not strongly envy any other agents according to Observations \ref{envy agents}, \ref{champ agents} and \ref{others}. This concludes the proof of Lemma \ref{efx}.
\end{proof}


\begin{lemma}\label{potential func u2}
	Rule $\textsf{U}_2$ is $\Phi$-improving.
\end{lemma}
\begin{proof}
	Let $i\in S_{\allocs'}-S_{\allocs}$. Then there exists a path from some agent $j\in S_{\allocs}$ to $i$. By Observation \ref{sources are min}, $\valu_j(\alloc_j)<\valu_i(\alloc_i)\leq \valu_i(\alloc'_i)$. Therefore, using Observation \ref{utility Change} and Lemma \ref{lex2}, we can conclude that $\Phi(\allocs') \lexlarger \Phi(\allocs)$.
	\HA{See the current statement of Lemma \ref{lex2}. You should argue more why the preconditions hold.}
\end{proof}

==> U3-prim.tex <==
\subsubsection*{Rule $\mathsf{U}_3$ \HA{Do we really need $\mathsf{U}_3$?}} 
Rule $\textsf{U}_3$ is a novel updating rule which is fundamentally different from the previous updating rules. In contrast to the former rules, after applying $\mathsf{U}_3$,  $\allocs$ Pareto dominates $\allocs'$. However, as we show in Lemma \ref{U3.3}, Rule  $\textsf{U}_3$ is $\Phi$-improving.

\vspace{0.5cm}
\begin{tcolorbox}[%colback=blue!5,coltitle=blue!50!black,colframe=blue!25,
	title= \textbf{Rule $\mathsf{U}_3$}]
	
	{Preconditions:}\label{pre1}
	\begin{itemize}
		\item $\sigma=(X, R)$ is a \goodalloc envy-decomposition.
		\item There exists a good $ \good \in P$ and a representative agent $r_\ell$ such that $v_{r_\ell}(g) = v(g)$
		\item Rules $\mathsf{U}_0$ and $\mathsf{U}_2$ are not  applicable.
	\end{itemize}
	\hrulefill
	
	{Guarantees:}
	\begin{itemize}
		\item $\sigma' = (X', R')$ is a \goodalloc envy-decomposition.
		\item $\Phi(\sigma')\lexlarger \Phi(\sigma)$.
	\end{itemize}
	\hrulefill
	
	{Process:}
	\begin{itemize}
		\item Allocate $g$ to $r_\ell$.
		\item Remove all wasted goods.
		\item Apply envy elimination on $X$.
	\end{itemize}
\end{tcolorbox}
\vspace{0.5cm}


\begin{corollary}[of Lemma \ref{extended-props}]\label{good-alloc-3}
	Let $\sigma' = (X', R')$ be the result of updating $\sigma = (X, R)$ via Rule $\textsf{U}_3$. Then, $\sigma'$ is a good envy-decomposition.
\end{corollary}

\iffalse
\begin{observation}
	If Rule $\mathsf{U}_3$ is applicable and $v_{r_\ell}(g) = v(g)$, then there exists an agent $j \in R_k$ for $k < \ell$, such that $j$ is an extended champion of $X_i \cup \{g\}$.
\end{observation}
\begin{proof}
	\todo{...}
\end{proof}
\fi
\begin{lemma}\label{subset-sources-t}
	Let $X'$ be the allocation after updating $X$ via Rule $\textsf{U}_3$. For every $1 \leq k < \ell$ and every agent $i \in R_k$, 
	\begin{itemize}
		\item if $i \in R'_t$, then $v_{r'_t}(X'_{r'_t}) \leq v_{r_k}(X_{r_k})$, and
		\item if $i \notin \{r_1, r_2, \ldots, r_{|R|}\}$, then $i \notin \{r'_1, r'_2, \ldots, r'_{|R'|}\}$.
	\end{itemize}
\end{lemma} 
\begin{proof}
	\HA{This is exactly like the proof of Lemma \ref{subset-sources-1}.}
	The proof is by induction on the distance of $i$ from $r_k$. If $i = r_k$, then either $i \in \{r'_1, \ldots, r'_{|R'|}\}$ and $v_{r'_t}(X'_{r'_t}) = v_{r_k}(X_{r_k})$ or, $v_{r'_t}(X'_{r'_t}) < v_{r_k}(X'_{r_k}) \leq v_{r_k}(X_{r_k})$. Now assume $i \neq r_k$, and $j$ is the preceding node of $i$ in a shortest path from $r_k$ to $i$ in $H_\sigma$. By induction assumption, $j \in R'_t$ for $v_{r'_t}(X'_{r'_t}) \leq v_{r_k}(X_{r_k})$. 
	The bundle of $i$ is not changed before the envy elimination. We have $v_i(X_i) > v_{r_k}(X_{r_k}) \geq v_{r'_t}(X'_{r'_t})$ and $v_j(X_i) = v(X_i)$. Therefore, either $i$ is added to some $R'_{t'}$ for $t' \leq t'$ or $i$ is added to $R'_t$.
\end{proof}
\begin{lemma}\label{U3.3}
	Rule $\textsf{U}_3$ is $\Phi$-improving.
\end{lemma}
\begin{proof}

\end{proof}

==> nOver2-intro.tex <==
In this section, we present an algorithm that leaves aside at most $\floor{n/2}-1$ many goods and finds an $\EFX$ allocation for the rest of the goods. The structure of our method is similar to the previous section: we start with an empty allocation $X$ and refine $X$ via a sequence of updating rules until none of the rules is applicable. These rules are designed in a way that guarantees the $\EFX$ property after each update. Our algorithm consists of four updating rules. 
Among these rules, the first three rules are similar to the updating rules introduced by Chaudhury \textit{et al. }\cite{charity}.
These rules are applicable as long as the number of remaining goods is at least the number of the sources in the $G_X$. However, since the number of the sources in the envy-graph might be as large as $n$, these rules only guarantee that the number of discarded goods is less than $n$. In our algorithm, we introduce another updating rule which is useful when the number of remaining goods is at least $\floor{n/2}$ and none of the former rules is applicable. 

Let us briefly discuss the idea behind our new updating rule. Let  $\{i_1,i_2,\ldots,i_k\}$ be the set of the sources in $G_X$ at some step of the algorithm, and for every $1 \leq \ell \leq k$ define $R_{i_\ell}$ as follows:
$$
	R_{i_\ell} = \{j|j \mbox{ is reachable from } i_\ell \} \setminus \bigcup_{\ell'<\ell} R_{i_{\ell'}}.  
	$$
The idea is that if $k > \floor{n/2}$, for at least one of the sources $i_\ell$  we have $R_{i_\ell} = \{i_\ell\}$. 
Given that none of the former updating rules is applicable, our new updating rule finds such a source $i_\ell$, allocates one good to her and then removes a subset of goods from $\alloc_{i_\ell}$ so that no agent strongly envies her. However, this modification might violate the $\EFX$ property since $i_\ell$ may strongly envy other agents after losing a subset of goods. If so, we continue removing goods from other bundles until the $\EFX$ property is restored. 

Note that, after this update, the utility of each agent either decreases or remains intact.  This may raise a question about the termination of our algorithm. Fortunately, we present a potential function $\Phi(X)$ and show that the value of $\Phi(X)$ increases after each update. To define such a potential function, we take advantage of the fact that after applying the above updating rule, the set of new sources in the envy-graph is a strict subset of the old ones. Indeed, assuming $S_{\alloc} = \{i_1,i_2,\ldots,i_k\}$ is the set of the source nodes such that $\util_{i_1}(\alloc_{i_1}) \leq \util_{i_2}(\alloc_{i_2}) \dots \leq \util_{i_k}(\alloc_{i_k})$, we define $\Phi(\alloc)$ as follows:
\begin{equation}\label{phi}
	\Phi(X) = \bigg[ \util_{i_1}(\alloc_{i_1}), \util_{i_2}(\alloc_{i_2}), \ldots, \util_{i_k}(\alloc_{i_k}),+\infty, \frac{1}{\sum_{i \notin S_X} |\alloc_{i}|}, \sum_{i \in S_X} |\alloc_{i}| \bigg],
\end{equation}
where $|\alloc_i|$ is the number of goods in the bundle of agent $i$. We show that after each update, $\Phi(X)$ increases lexicographically~\footnote{
	%We say vector $v=[v_1,\ldots,v_r]$ is lexicographically smaller than vector $v'=[v'_1,\ldots, v'_{r'}]$, if  either there exists some $j\leq r$ such that for all $i< j, v_i= v'_i$ and $v_j<v'_j$ or $r<r'$ and for all $1 \leq i \leq r$ we have $v_i=v'_i$. 
	We say vector $\textbf{v}=[\textbf{v}_1,\ldots,\textbf{v}_r]$ is lexicographically larger than vector $\textbf{v}'=[\textbf{v}'_1,\ldots, \textbf{v}'_{r'}]$ or $\textbf{v} \lexlarger \textbf{v}'$, if  either there exists some $j\leq \min\{r, r'\}$ such that for all $i< j, \textbf{v}_i= \textbf{v}'_i$ and $\textbf{v}_j>\textbf{v}'_j$ or $r>r'$ and for all $1 \leq i \leq r'$ we have $\textbf{v}_i=\textbf{v}'_i$.}
and therefore the algorithm eventually ends after a finite number of updates. 


%Therefore, any potential 
%
%Although  it does not seem that this modification is improving in any front, we suggest a potential function which increases after all the updates, including the above update. To find such a potential function, we take advantage of the fact that after applying the above updating rule, the set of new sources is a strict subset of the old ones. 

%modifies the bundle of a single source in a way that the value of this source for her bundle drops but someone starts to envy her.
%The idea is to start with an empty allocation and apply some updating rules that gauranty $\EFX_0$ and ultimately allocate all the goods except at most $\floor{n/2}$ of them. Similar to \cite{charity}, our updating rules take a pair $(X, P)$, where $X$ is the current allocation and $P$ is the set of unallocated goods and then return another pair $(X', P')$. We redefine and slightly modify the updating rules in \cite{charity}. These updating rules are applicable as long as the number of unallocated goods is larger than or equal to the number of the sources in the envy-graph. We also introduce a new rule which is surely applicable in case the the number of sources in the envy-graph is more than $\floor{n/2}$ and the other rules are not applicable. Together with the former updating rules, we can improve the allocation as long as the number of unallocated goods is larger than $\floor{n/2}$. 

%For a closer look at our new updating rule, let $\agent_1, \dots, \agent_s$ be the sources of the current envy-graph and $R_i$ be the agents reachable from $\agent_i$ and not reachable from any $\agent_j$ for $j < i$. We refer to the sources $\agent_i$ with $R_i = \{\agent_i\}$ as single sources. We prove that an updating rule is applicable if a single source exists. By pigeonhole principle, if the number of sources is larger than $\floor{n/2}$, a single source exists. Our new updating rule modifies the bundle of a single source in a way that the value of this source for her bundle drops but someone starts to envy her. Hence, she is not a source in the new allocation anymore. More follow-up modifications might be required to maintain $\EFX_0$ property of the allocation. All these modifications reduce the utility of some agents for their bundles. Although it does not seem that the allocation is improving in any front, the technical novelty of our contribution is to come up with a potential function which increases after each update. We take advantage of the fact that after applying our new updating rule, the set of new sources is a strict subset of the old ones. 

%In order to prove that our algorithm actually terminates, we define a simple but sophisticated potential function $F$, which is always increasing after applying each updating rule. Unlike in \cite{charity}, in our algorithm, an updating rule might decrease the social welfare. In order to find an always-improving pattern in our updating rules, we restricted our attention to the sources of the current envy-graph. We prove that the utility profile of the sources appended with a large number, never decreases lexicographically. In case this value does not strictly increase, the number of goods allocated to the sources increases. Formally, $F(\allocs, P)=((u_1(\alloc_1), \dots , u_s(\alloc_s), +\infty), |M_S|)$ is always increasing, where $(u_1(\alloc_1), \dots , u_s(\alloc_s))$ is the utility profile of the sources and $M_S$ is the set of goods allocated to the sources. Therefore, the algorithm terminates.


\begin{example}
	Let $N=\{1, 2, 3\}$, $M=\{\good_1, \good_2, \good_3, \good_4, \good_5, \good_6\}$ and assume that the current allocation is $\alloc_1 = \{\good_1, \good_2\}$, $\alloc_2 = \{\good_3\}$, $\alloc_3 = \{\good_4, \good_5\}$ and $\good_6$ is not allocated. Also, suppose that the valuations are as shown in Figure~\ref{graph-before-after}. The envy-graph of this instance before the update is also depicted in Figure \ref{graph-before-after}(a) and agents $1$ and $3$ are the source nodes. Therefore we have, 
	\begin{align*}
		\Phi(\allocs) &= [\util_1(\alloc_1), \util_3(\alloc_3), +\infty, \frac{1}{|\alloc_2|} ,|\alloc_1|+|\alloc_3|]\\
		&= [6,9, +\infty, 1,4].\\
    \end{align*}
    We remark that for this instance, the only applicable updating rule is $\textsf{U}_3$. This rule allocates $\good_6$ to agent $3$ and takes back good $\good_5$ from her. Figure \ref{graph-before-after}(b) shows the envy-graph after the update. Let $X'$ be the allocation after the update. We have
    \begin{align*}
		\Phi(\allocs')&= [\util_1(\alloc'_1),+\infty, \frac{1}{|\alloc'_2|+|\alloc'_3|},|\alloc'_1|] \\ 
		&= [6,+\infty, \frac{1}{3},2].
	\end{align*}
	Hence,
	$$
		\Phi(\allocs') \lexlarger \Phi(\allocs).
	$$
\end{example}
\begin{figure}%[H]
	\centering
		\begin{subfigure}{8cm}
		\centering
		
		\begin{tabular}{ c|c c c c c c}
			& $\good_1$ & $\good_2$ & $\good_3$ & $\good_4$ & $\good_5$ & $\good_6$\\
			\hline
			$\util_1$& \fbox{$1$} & \fbox{$5$} & $7$ & $0$ & $0$ & $0$\\
			$\util_2$& $0$ & $5$ & \fbox{$7$} & $4$ & $0$ & $4.5$\\
			$\util_3$& $0$ & $5$ & $0$ & \fbox{$4$} & \fbox{$5$} & $4.5$\\
		\end{tabular}
		\vspace{1cm}
		
		\begin{tikzpicture}[
		sourcenode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
		node/.style={circle, draw=black!60, fill=white!5, very thick, minimum size=5mm},
		]
		%Nodes
		\node[sourcenode]      (maintopic)                              {$1$};
		\node[node]      (rightsquare)       [right=of maintopic] {$2$};
		\node[sourcenode]        (lowercircle)       [below=of maintopic] {$3$};
		
		%Lines
		\draw[->] (maintopic.east) -- (rightsquare.west);
		%\draw[->] (rightsquare.south) .. controls +(down:7mm) and +(right:7mm) .. (lowercircle.east);
		\end{tikzpicture}
		\vspace{0.25cm}
		\\(a)
	\end{subfigure}
	\begin{subfigure}{8cm}
			\centering
			\begin{tabular}{ c|c c c c c c}
			& $\good_1$ & $\good_2$ & $\good_3$ & $\good_4$ & $\good_5$ & $\good_6$\\
			\hline
			$\util_1$& \fbox{$1$} & \fbox{$5$} & $7$ & $0$ & $0$ & $0$\\
			$\util_2$& $0$ & $5$ & \fbox{$7$} & $4$ & $0$ & $4.5$\\
			$\util_3$& $0$ & $5$ & $0$ & \fbox{$4$} & $5$ & $\fbox{4.5}$\\
		\end{tabular}
		\vspace{1cm}\\
			\begin{tikzpicture}[
		sourcenode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
		node/.style={circle, draw=black!60, fill=white!5, very thick, minimum size=5mm},
		]
		%Nodes
		\node[sourcenode]      (maintopic)                              {$1$};
		\node[node]      (rightsquare)       [right=of maintopic] {$2$};
		\node[node]        (lowercircle)       [right=of rightsquare] {$3$};
		
		%Lines
		\draw[->] (maintopic.east) -- (rightsquare.west);
		\draw[->] (rightsquare.east) -- (lowercircle.west);
		\end{tikzpicture}
\vspace{2cm}
				\\(b)
	\end{subfigure}
	\caption{(a) Envy-graph of allocation $\allocs$ (before the update), (b) Envy-graph of allocation $\allocs'$ (after the update).}
	\label{graph-before-after}
\end{figure}


%Let us remark that the term $\frac{1}{\sum_{i \notin S_X} |\alloc_{i}|}$ in Equation \eqref{phi} is not necessary for the updating rules in this section to improve $\Phi$. Formally speaking, for 
%$$
%\Phi'(X) = \bigg[ u_{i_1}(\alloc_{i_1}), u_{i_2}(\alloc_{i_2}), \ldots, u_{i_k}(\alloc_{i_k}),+\infty, \sum_{i \in S_X} |\alloc_{i}| \bigg],
%$$
%all the updating rules in this section increase $\Phi'$ lexicographically. However, in Section \ref{ef2x}, we introduce another updating rule for which the term $\frac{1}{\sum_{i \notin S_X} |\alloc_{i}|}$ is crucial to improve $\Phi$.

%\begin{table}%[H]
%	\centering
%	\begin{tabular}{ c|c c c c c c}
%		& $\good_1$ & $\good_2$ & $\good_3$ & $\good_4$ & $\good_5$ & $\good_6$\\
%		\hline
%		$\util_1$& \fbox{$1$} & \fbox{$5$} & $7$ & $0$ & $0$ & $0$\\
%		$\util_2$& $0$ & $5$ & \fbox{$7$} & $4$ & $0$ & $4.5$\\
%		$\util_2$& $0$ & $5$ & $0$ & \fbox{$4$} & \fbox{$5$} & $4.5$\\
%	\end{tabular}
%	\caption{Utility function of the agents for the goods and the allocation $\allocs$ (before the update)}
%	\label{before}
%\end{table}

==> update-rules-intro.tex <==
%Our algorithm consists of $4$ updating rules. Starting with an empty allocation, as long as an updating rule is applicable, we apply it. If no updating rule is applicable, the algorithm terminates.

Throughout  this section we introduce our updating rules. As mentioned, our algorithm consists of four updating rules $\textsf{U}_0,\textsf{U}_1,\textsf{U}_2,$ and $\textsf{U}_3$.
We dedicate a section to each updating rule which precisely describes its preconditions, guarantees, and the updating process itself. These rules are designed in a way that the allocation satisfies the following properties during the algorithm:

\begin{itemize}
	\item $\bf{\EFX}$: the allocation remains \textbf{$\EFX$} during the algorithm.
	\item \textbf{Almost non-wastefulness}: %for all non-source agents $\agent$, $\util_\agent(\alloc_\agent) = \valu(\alloc_\agent)$. In other words, 
	each good allocated to a non-source agent is not wasted.% has a non-zero value to her. 
\end{itemize}

For convenience, in this section $X$ refers to the allocation before the update and $X'$ refers to the allocation after the update. Given that the above properties always hold, by Corollary \ref{DAG} we have that the envy-graph is always acyclic. Moreover, our updating rules have the property that they always increase $\Phi$ lexicographically, i.e., after each update, we have $\Phi(X') \lexlarger \Phi(X)$. 
We call such a property $\Phi$-improving. 

 

%Note that at any point, if the graph of an allocation is not a DAG, we can remove its directed cycles and the resulting allocation is still $\EFX$. %We call a vertex of a DAG source, when it has no incoming edges. 

